Rossby Wave Instability and Substructure Formation in 3D Non-Ideal MHD Wind-Launching Disks

Rings and gaps are routinely observed in the dust continuum emission of protoplanetary discs (PPDs). How they form and evolve remains debated. Previous studies have demonstrated the possibility of spontaneous gas rings and gaps formation in wind-launching disks. Here, we show that such gas substructures are unstable to the Rossby Wave Instability (RWI) through numerical simulations. Specifically, shorter wavelength azimuthal modes develop earlier, and longer wavelength ones dominate later, forming elongated (arc-like) anti-cyclonic vortices in the rings and (strongly magnetized) cyclonic vortices in the gaps that persist until the end of the simulation. Highly elongated vortices with aspect ratios of 10 or more are found to decay with time in our non-ideal MHD simulation, in contrast with the hydro case. This difference could be caused by magnetically induced motions, particularly strong meridional circulations with large values of the azimuthal component of the vorticity, which may be incompatible with the columnar structure preferred by vortices. The cyclonic and anti-cyclonic RWI vortices saturate at moderate levels, modifying but not destroying the rings and gaps in the radial gas distribution of the disk. In particular, they do not shut off the poloidal magnetic flux accumulation in low-density regions and the characteristic meridional flow patterns that are crucial to the ring and gap formation in wind-launching disks. Nevertheless, the RWI and their associated vortices open up the possibility of producing non-axisymmetric dust features observed in a small fraction of protoplanetary disks through non-ideal MHD, although detailed dust treatment is needed to explore this possibility.

==> Discussion.tex <==
% very short discussion is sufficient

An interesting question to address in future investigations is how RWI affects the {\it dust} distribution and the disk appearance in continuum emission. Most observed disk dust substructures appear axisymmetric, although a small fraction shows non-axisymmetric features, including arcs, which are potentially vortices. The RWI vortices discussed in this paper open up the possibility of producing such dusty vortices in non-ideal MHD wind-launching disks. However, detailed dust treatment is needed to explore this possibility quantitatively. The current simulation will also benefit from adaptive (rather than static) mesh refinement, which will better resolve the vortices formed in the global 3D simulations. 


%Short Discussion
%{\color{violet}We investigate the case starting with the initial pressure bump (T-3D-2000) and the case starting with the hydro equilibrium state (T-3D-0), and the Rossby waves are unstable on both cases in the magnetized disks. The non-axisymmetric structures may be generated by these unstable wave modes. }
%\subsection{Relatively rare non-axisymmetric structures in the Observation} \label{subsec:rare_non_axisymmetric_observation}
%{\color{violet}The observations of the PPDs, however, only find a $\sim$ 25 $\%$ of targets that have non-axisymmetric substructures \cite[e.g.,][]{Armitage19}. The measurement of the gas distribution at a high resolution would be challenged because of the optical depth effects and chemical variation. But still, the observational evidence via the dust continuum emission, such as the ALMA Large Program 'eDisc', can measure high-resolution dust continuum emission to understand the dust distribution. The dust rings and gaps are relatively axisymmetric in most of the observations. On the other hand, our investigations of the Rossby wave stability in the magnetized disk show the RWI may naturally develop anywhere (see Fig. \ref{fig:RWI_2D}) and the $m=1$ mode may show the prominent non-axisymmetric vortex structure in the PPDs. Model T-3D-2000 tells a similar story to previous studies of RWI in the PPDs in that the most unstable mode first shows the pattern, and the $m=1$ mode finally dominates the system to form a prominent vortex \cite[e.g.,][]{Meheut12,Richard13,Ono18}. Our simulations, however, include the stratified disk, and the disk winds strongly influence the vertical structure that may change the gas flow on top and bottom of the vortex which may have a negative effect on the vortex survival (also see the text in \S\ref{sec:results}). Fig. \ref{fig:LateTimeModes} b shows the $m=1$ can show the prominent non-axisymmetric structure but it might decay in the later time. 

%The other explanation to illustrate the opposite between the observations and our results is the pressure bump amplitude in nature may not high as in our simulations. Note that the mechanism to generate ring and gap formation in the magnetized disk is disk wind-driven accretion to distribute the gas distribution. The accretion rates in our simulation are $\sim 10^{-5}-10^{-6} M_{\bigodot}/{\rm year}$. The accurate accretion rate in the Case II phase is still debated but the accretion rates in our simulation are seen to be likely in the Case 0 phase. The higher accretion rate can generate a stronger separation between rings and gaps, and the RWI can easily develop in the environment has a higher amplitude difference between the rings and gaps. If the accretion rate is $\sim 10^{-8} M_{\bigodot}/{\rm year}$, we can expect the amplitude of the pressure bumps between rings and gaps may lower than what we get in the simulation, and the RWI may not robust to form significant non-axisymmetric structures. Based on the above discussion, we believe
}
%{\color{red}
%the $m=1$ may be observable in principle (but not likely in practice given its short lifetime) unless it is kept alive by the ring/gap formation mechanism itself! 
%}
%{\color{violet} This may partially explain the reason why the observed non-axisymmetric substructures are rarer than the axisymmetric rings and gaps.}

%\subsection{Future refinements} \label{subsec:future_work}

%{\color{red}
%Future direction: AMR (rather than SMR) may be needed to resolve the vortices better. 
%}
%{\color{violet} There are several directions to move forward to pursue this ring and gap formation investigation. First of all, the adapted mesh refinement (AMR) technique can be applied to resolve the vortices in the disk better. The spatial resolution in our results isn't as good as the previous 2D vortex studies, particularly, in the radial direction. The other possible direction is that includes the lived dust in our simulation. It is not clear whether the dust can clump in the RWI-triggered vortices even if the \cite{Zhu14_dust} shows particles may concentrate at planete-induced vortices. Particularly, there are strong meridian vortices in our disk, and the dust motion may be highly influenced by these meridian vortices. Furthermore, the Hall effect should be included in the induction equation in future work. The Hall effect can play an important role in transporting magnetic flux to the outer orbit that leads to vertical magnetic field configuration in the mid-plane region \cite[e.g.,][]{Bae17}. \cite{Bae17} shows the flux transport rate increases with increasing disk magnetization, and the disks in our cases with the chemical table are well-coupled to the magnetic field. It is crucial to understand whether the Hall effect plays a role in stabilizing the Rossby wave in the wind-launching disk.

%}

==> Discussion_old.tex <==
% Discussion

We investigate the fluid properties in a series of non-ideal MHD simulations, treating the charge densities using a power-law prescription and a simple chemistry model including dust grains. 
The chemical network's parameters are chosen to yield a relatively large Elsasser number $\Lambda > 1$, which facilitates the formation of rings and gaps in PPDs   \citep[e.g.][]{Nolan23}. 
In Section \S \ref{sec:dust}, we include the post-processing dust particles to study the dust motion in the magnetized disk. 
We present both meridian and equatorial slices of the 3D PPDs with dust particles superposed to 
illustrate the gas dynamics and corresponding dust behaviors (see Fig.~\ref{fig:dv_column} and \ref{fig:overlap_dust}). 

\subsection{The vortex and dust motion} \label{subsubsec:discussion_for_vortex_dust_motion}


\cite{Lyra15} noted that the RWI is the form of the Kelvin-Helmholtz instability in differentially rotating disks, with the surplus shear converted into vorticity.
\cite{Li2000} gives linear RWI. 
\cite{Lehmann22} figure 18 also shows the vortex. 

compare with \citet{Cui21}

We find that dust particles are trapped between the vortices, and this result agrees with \cite{Hu22}'s 2D non-ideal MHD simulation with live particles. 
\cite{Hu22} shows that most large grains are trapped in the super-Keplerian regions, while some smaller dust grains can stay in the sub-Keplerian regions. 
This agrees with our 3D simulation (see Figure \ref{fig:dv_column}, a slice through the meridian plane). 

We observe that large-scale disk winds may be developed from a superposition of the nonlinear waves generated by the accretion flow and surface velocity shear.
Previous studies have found that the magnetized wind drives the disk accretion \citep[e.g.][]{Bai13, Takahashi18, Lesur21}. 
However, we see the inverse: the accretion flow-triggered turbulence drives the launch of winds from the disk in our 3D simulation.
The accretion flow signifies strong disk dynamics, facilitating the formation of rings and gaps.
As a result, rings and gaps appear almost simultaneously as the large-scale disk winds are launched. 

In addition to the meridian plane ($r,\theta$), we also examine the gas dynamics by RWI-triggered vortices and resulting dust motion in the equatorial plane ($r,\phi$).
The linear theory put forward by \cite{Lovelace99} predicts that the peaks of the column density are aligned with the regions with vertical vorticity in the mid-plane, and it agrees with our model (see Figure \ref{fig:overlap_dust}).
The post-processing dust distribution is in between the high column density and the low column density regions.
Dust concentration between the vortices in opposite directions may increase the frequency of collisions and favor grain growth. 
Moreover, the dust concentration arises naturally without introducing an artificial global pressure bump, so the streaming instability can be triggered self-consistently \citep[e.g.][]{Youdin05}. 

We investigate vorticities of both meridian and equatorial planes and find that the $\phi$ direction vorticity in the meridian plane is one order of magnitude larger than the vertical direction vorticity in the mid-plane. 
%Figure 4 of \cite{Hu22} shows the smaller grains drift away more easily from the mid-plane.
%Considering the size distribution in the real PPDs, 
The motion of most grains is affected more by the $\phi$ direction vorticity in the meridian plane than the vertical direction vorticity. 
Larger grains are concentrated in the super-Keplerian regions as a result of their interaction with the $\phi$ direction vortices. However, smaller dust grains can still populate sub-Keplerian regions because their motion follows the gas.
Because the vortices are weaker in the sub-Keplerian regions, the smaller dust grains can concentrate around the mid-plane, where they can be affected by the RWI-triggered vortices. 
Thus, the RWI-triggered vertical vortices are still important to dust dynamics and ring and gap formation in PPDs. 

%Furthermore, these vortex structures may drive the currents to affect the magnetic flux transportation, which is important to the disk dynamics.

\subsection{Connect to observations} \label{subsec:discussion_for_observations}

Rings and gaps have been frequently detected in class II
protoplanetary objects by dust emission \citep[e.g.][]{ALMA15, Andrews18}. 
However, the gas motion cannot be resolved using current telescopes. 

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{Figures/test_rotate_phi_dust_t1000_low_resolution.png}
    \caption{
    Snapshots of (a) the gas column density and (b) the estimated dust column density at $t=1000$ yr. The estimated dust column density is defined as summing up all the dust particles in the $\theta$ direction and divided by the ratio of the one percent of the initial disk mass to the number of the initial dust particles. {\color{red} [Chun-Yen: Please fix the issue of one side of the disk appearing bigger than the other side, perhaps by putting the disk at a very large distance from the camera.]}
    {\color{brown} purpose: give a sense that dust is misaligned with the gas.
    Do we still use an oval-shaped plot?}
    {\color{red} low resolution}
    }
    
    \label{fig:dust_column_rotate}
\end{figure*}

Figure \ref{fig:dust_column_rotate} shows the snapshots of the gas column density in panel (a) and the corresponding estimated post-processing dust column density in panel (b). 
There are 4 million post-processing dust particles included in the model. 
We estimated the mass each dust grain represents by assuming the dust carries one percent of its local gas mass. 
Then, we estimated the dust column density by integrating the dust mass density over the $\theta$ direction. 
The gas column density plot clearly shows non-axisymmetric substructures triggered by the RWI, while the dust column density doesn't show the same substructure pattern as the gas.
We point out that the dust distribution is offset from the gas in radius and azimuthal directions in \S \ref{sec:results}.
Thus, even if observers detect axisymmetric dust rings and gaps using the dust continuum emission, the gas in the PPDs is not necessarily axisymmetric. 
We emphasize the possibility that the non-axisymmetric gas substructure could drive vortices to influence the dust motion.
Nevertheless, the dust with different particle sizes will have different drag forces with the gas, resulting in different speeds and positions of the dust. 
In the future, we may include a more realistic grain size distribution in our PPD models. 


\begin{comment}
\subsection{particle clump}
1. test Xiao method
\begin{align}
 & v_{\rm d} = \vel - \delta v
\end{align}

2. test streaming instability equilibrium state
\begin{align}
 & v_{\rm dx} = - \frac{2 \tau_s}{(1+\epsilon)^2 + \tau^2} \eta R_0 \Omega_0
 & v_{\rm dy} = - \frac{\epsilon +1}{(1+\epsilon)^2 + \tau^2} \eta R_0 \Omega_0
\end{align}

\subsection{facility to the dust concentrate}
streaming instability \citet{Youdin05}
some other dust concentrate 
\citet{Hsu22}
\cite{Li19} limitation for streaming instability. 
McKinney, black hole simulation. 


%\begin{figure*}
%    \centering
%    \includegraphics[width=\linewidth]{Figures/column_with_dust_t1000.png}
%    \caption{
%    caption
%    }
%    \label{fig_column_with_dust}
%\end{figure*}
\end{comment}

==> dust.tex <==
% 3D_From_Start
 
{\color{red}
Hint: be careful of the initial dust position.
}

%\begin{figure*}
%    \centering
%    \includegraphics[width=\linewidth]{Figures/Paper_column_rz_rphi.png.jpg}
%    \caption{
%    caption
%    }
%    \label{fig_column_rz_rphi}
%\end{figure*}

We use a post-processing code to trace dust trajectory in the magnetized disk. The code is described in Tu et al. (2024, submitted) and discussed briefly in Appendix \ref{sec:appendix_b_dust}, which includes a comparison between the dust distributions computed using active particles evolved together with gas and through post-processing. The benefit of the post-processing method is that we can include a much larger number of particles for 3D simulations with available computational resources. 

\subsection{Dust Distribution through Post-Processing}

\subsection{Dust post-processing} \label{subsec:pros_processing_dust}

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{Figures/test_dv_column_hydro_dust_slice_with_curlV_t1000.png}
    \caption{
    Snapshots of (a) $\phi$ average of the fraction difference between the gas rotation speed and the local Keplerian speed with $\phi$ integral of 1mm size post-processing dust, (b) the column density in the logarithmic scale (black) and the vertical magnetic field strength (red) in the mid-plane, and (c) the mass density in the logarithmic scale (black) and the vorticity (red) in the mid-plane at $t=1000$ yr. The super-Keplerian regions (red) concentrate more dust than the sub-Keplerian regions (blue). The color of the post-processing dust is noted by the initial ($t=0$) position, which is plotted as red (initial at 1 au) to blue (initial at 50 au). Panel (a) shows the post-processing dust follows the accretion flow to migrate to the inner region and is trapped in the super-Keplerian regions. Panel (b) indicates the column density is anti-correlated to the vertical magnetic field strength. Panel (c) shows the local peaks of the vorticity in the mid-plane are aligned with the local peaks of the gas mass density. 
    {\color{brown} purpose: give a radial profile of the dust population corresponding to the superKeplerian regions. vorticity has the same phase as column density.
    Maybe think about how to make the plot more pretty.}
    }
    \label{fig:dv_column}
\end{figure*}

For the post-processing, we choose a grain size of $s=1$~mm and place 4 million particles in $\pi/2 - 0.1<\theta<\pi/2 + 0.1$ with proportionally more particles in denser gas regions. 
Figure \ref{fig:dv_column} shows the positions of the dust particles and the fractional difference between the gas rotation speed and the local Keplerian speed at $t=1200$~yr {\color{red} [Please use consistent time, $t=1200$~year for this section.]}. 
The colors of the dust particles are determined by their initial positions, varying from red (with initial positions near $r \sim 1$ au) to blue (with initial positions near $r \sim 50$ au).
In the meridian plane, super-Keplerian regions (red) trap more 1~mm-sized dust than the sub-Keplerian regions (blue). 
The dust in the PPDs generally migrates to the inner part of the disk due to the accretion flow. {\color{red} This accretion is dominated by a thin warped current sheet in 3D, as in the 2D case (e.g., Suriano et al. 2019; Xiao et al. 2022) [Chun-Yen: Is this true? This will be hard, but would it be possible to get the 3D shape of the locations of the fastest accretion (with the most negative $\rho v_r$ inside the disk at a given pair of $r,\phi$ but different $\theta$; we can talk about this on Tuesday if this is not clear to you]. Dust settles to this accretion sheet and is advected inward toward the inner edge of a ring where the rotation speed is super-Keplerian. There, part of the accretion stream is forced by the strong poloidal magnetic field in the gap interior to the ring to move away from the midplane and then circulate backward toward larger radii, carrying the dust along with it. The meridional gas circulation and dust vertical settling towards the midplane combine to concentrate dust near the inner super-Keplerian part of the ring. [Chun-Yen: This is the mental picture based on Xiao's 2D simulation; is this picture still true in 3D? If not, what are the differences and why? Does RWI modify this picture at all?]}. 

{\color{red} Panel (b) of Figure \ref{fig:dv_column} shows the column density normalized by its initial value (black) and the vertical magnetic field strength normalized by its initial value (red) on the mid-plane. 
}
The column density is inversely correlated with the poloidal field strength, with stronger magnetic fields in the gaps than in the rings. A comparison between panel (a) and panel (b) shows that the peaks of the gas column density (rings) are misaligned with the super-Keplerian regions, which is consistent with the above picture that advection by gas motions affects the dust distribution than the gas density. Figure \ref{fig:dv_column} (c) shows the mass density normalized to its initial value (black) and the total vorticity (including all three components; red) normalized by the local Keplerian frequency on the mid-plane. The vorticity is correlated with the mass density; in particular, the vorticity's local peaks are aligned with the mass density's local peaks
{\color{red} [This is interesting; which component of vorticity dominates?].
\cite{Lovelace99}'s linear theory relates the column density and the vorticity as parameters of the RWI's eigenfunction. 
A similar relation between the vorticity profile and the column density profile in panel (b) can be seen. [I am not sure what these two sentences mean.] }

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{Figures/dust_overlap_Curl_V_R_phi_t1200_low_resolution.png}
    \caption{
    Snapshots of the (a) face on view of the column density with vertical vorticity in the mid-plane at the orbit $r=$ 15-17 au (panel b), 20-23 au (c), 27-30 au (d), and 35-39 au (e) including 1~mm sized post-processing dust (pink dots) at $t=1200$ yr. Note that we limit the column density in the logarithmic scale to the given values to emphasize vortices in the plot.
    Panels (b) and (c) show the saturated state of the vortices, and the highest column density regions correspond to the negative vorticity parts. On the other hand, gap regions are consistent with positive vorticity regions. Panels (d) and (e) display the growth state of the vortices. Most post-processing dust is trapped between the vortices and the vorticity $\sim$ 0 regions. 
    {\color{brown} purpose: give a phi profile of the dust population corresponding to the vortices. Also, high beta regions? change to beta?
    Do we still need to plot the left-hand side circle plot?}
    {\color{red} low resolution version.}
    }
    \label{fig:overlap_dust}
\end{figure*}


Figure \ref{fig:overlap_dust} shows snapshots of the equatorial plane of the column density (panel a) and vertical vorticity overplotted by 1mm size dust (pink dots) in the mid-plane at $r=$ 15-17 au, 20-23 au, 27-30 au, and 35-39 au in panel b, c, d, and e, respectively at $t=1200$ yr. {\color{red} [Use normalized column density here to be consistent with other plots.]}
The negative (blue) and positive (red) streamline loops in panels (b) to (e) indicate the locations of clockwise and counter-clockwise vortices, respectively.
The clockwise vortices are located at the denser regions, and the counter-clockwise vortices correspond to the less dense gap regions.
Different orbits show the different states of the RWI in the disk.
Similar to Figure \ref{fig:curlV_slice}, the dynamics are still rapidly evolving and have not yet saturated beyond $r =$ 35 au.
Compared with panels (d) and (e), panels (b) and (c) have much fewer dust particles because of the gas sub-Keplerian motion in those regions (see Figure \ref{fig:dv_column}). 
The dust particles are concentrated where the vorticity is $\sim $ 0, the region between strong vortices. {\color{red} [The concentration is unclear to my eyes, so I am not sure it is true. If it is true, I am not sure why. Given that the dust concentration in 2D is driven by an interplay between advection by gas motions and vertical settling, I suspect the same is true in 3D. From this point of view, it is crucial to understand the accretion sheet in 3D, how this sheet is modified by RWI, and the relation between this sheet and the meridional circulation that lifts the dust away from the midplane. We may need to build a picture of dust distribution based on the 2D picture and how RWI modifies it, starting with how RWI modified the gas distribution and motions.]}
Note that Figure \ref{fig:overlap_dust} does not illustrate the vertical motion of the dust particles, so the dust particles' motion in 3D is not fully captured.  
Nevertheless, we can still observe the influences the vortices impose on the dust trajectory in the mid-plane. 
Because the dust particles are located between the vortices, the local peaks of the number density of the dust particles are not aligned with the maximum of the gas column density, which agrees with Figure \ref{fig:dv_column}. 

%{\color{violet}
%\subsection{axisymmetry structure}
%KH instability \citet{Miura82}
% Plot a t vs 3 different sizes concentration rates at different vorticity
%Plot a radial profile of vorticity vs t, to show the formation of rings and gaps at the similar time of disk wind
%Checking plasma beta in the ring and gap regions. See whether the magnetic field may affect the vortices}

==> table_ionize.tex <==
\begin{table}
\caption {
The cosmic ray ionization rates for the neutral species. Adapted from the Table 2 in \citep{Umebayashi90}
\label{ch_table_ionize}
} 
%\begin{ruledtabular}
\begin{tabular}{llllll}
  Reaction  & Rate \\
        \hline
  ${\rm H_2} \longrightarrow {\rm H_2}^+ + {\rm e}$ & 0.97$\xi$\\
  ${\rm H_2} \longrightarrow {\rm H}^+ +{\rm H} + {\rm e}$& 0.03$\xi$\\
  ${\rm He} \longrightarrow {\rm He}^+ + {\rm e}$&  0.84$\xi$\\

  & $\xi = 10^{-17} {\rm s^{-1}}$ 
\end{tabular}
%\end{ruledtabular}
\end{table}

==> table_reaction.tex <==
\begin{table}
\caption {
Reaction.
\label{ch_table_reaction}
} 
%\begin{ruledtabular}
\begin{tabular}{llllll}
  Reaction  & Rate coefficient (${\rm cm^3 s^{-1}}$) \\
        \hline
  ${\rm H}^+ + {\rm O} \longrightarrow {\rm O}^+ + {\rm H}$ & $7.0 \times 10^{-10} {\rm exp} (-232/T)$\\
  ${\rm H}^+ + {\rm O_2} \longrightarrow {\rm O_2}^+ + {\rm H}$ & $1.2 \times 10^{-9} $\\
  ${\rm H}^+ + {\rm Mg}   \longrightarrow {\rm Mg}^+   + {\rm H}$ & $1.1 \times 10^{-9} $\\
  
  ${\rm He}^+ + {\rm H_2}   \longrightarrow {\rm H}^+   + {\rm H} + {\rm He}$  & $1.5 \times 10^{-13} $\\
  ${\rm He}^+ + {\rm CO}    \longrightarrow {\rm C}^+   + {\rm O} + {\rm He}$  & $1.6 \times 10^{-9} $\\
  ${\rm He}^+ + {\rm O_2}   \longrightarrow {\rm O}^+   + {\rm O} + {\rm He}$  & $1.0 \times 10^{-9} $\\

  ${\rm H_3}^+ + {\rm CO}   \longrightarrow {\rm HCO}^+   + {\rm H_2} $  & $1.7 \times 10^{-9} $\\
  ${\rm H_3}^+ + {\rm O}    \longrightarrow {\rm OH}^+    + {\rm H_2} $  & $8.0 \times 10^{-10} $\\
  ${\rm H_3}^+ + {\rm O_2}  \longrightarrow {\rm O_2H}^+  + {\rm H_2} $  & $6.4 \times 10^{-10} $\\
  ${\rm H_3}^+ + {\rm Mg}    \longrightarrow {\rm Mg}^+     + {\rm H_2} + {\rm H}$  & $1.0 \times 10^{-9} $\\

  ${\rm C}^+ + {\rm H_2}   \longrightarrow {\rm CH_2}^+   + h\nu $     & $6.0 \times 10^{-16} $\\
  ${\rm C}^+ + {\rm O_2}   \longrightarrow {\rm CO}^+     + {\rm O} $  & $7.5 \times 10^{-10} $\\
  ${\rm C}^+ + {\rm O_2}   \longrightarrow {\rm O}^+     + {\rm CO} $  & $4.1 \times 10^{-10} $\\
  ${\rm C}^+ + {\rm Mg}     \longrightarrow {\rm Mg}^+     + {\rm C} $   & $1.1 \times 10^{-9} $\\

  ${\rm C}^+ + {\rm Mg}     \longrightarrow {\rm Mg}^+     + {\rm C} $   & $1.1 \times 10^{-9} $\\

  ${\rm CO}^+ + {\rm Mg}     \longrightarrow {\rm Mg}^+     + {\rm CO} $   & $2.9 \times 10^{-9} $\\
  ${\rm O_2}^+ + {\rm Mg}     \longrightarrow {\rm Mg}^+     + {\rm O_2} $   & $2.9 \times 10^{-9} $\\
  ${\rm OH}^+ + {\rm Mg}     \longrightarrow {\rm Mg}^+     + {\rm OH} $   & $2.9 \times 10^{-9} $\\
  ${\rm O_2H}^+ + {\rm Mg}     \longrightarrow {\rm Mg}^+     + {\rm O_2H} $   & $2.9 \times 10^{-9} $\\
  ${\rm HCO}^+ + {\rm Mg}     \longrightarrow {\rm Mg}^+     + {\rm HCO} $   & $2.9 \times 10^{-9} $\\
  ${\rm CH_2}^+ + {\rm Mg}     \longrightarrow {\rm Mg}^+     + {\rm CH_2} $   & $2.9 \times 10^{-9} $\\
  
  ${\rm H}^+ + {\rm e} \longrightarrow {\rm H} + h\nu$ & $3.5 \times 10^{-12} (300/T)^{0.7}$\\
  ${\rm He}^+ + {\rm e} \longrightarrow {\rm He} + h\nu$ & $4.5 \times 10^{-12} (300/T)^{0.67}$\\
  
  ${\rm H_3}^+ + {\rm e} \longrightarrow {\rm H} + {\rm H} + {\rm H}$ & $2 \times 10^{-8} $\\
  ${\rm H_3}^+ + {\rm e} \longrightarrow {\rm H_2} + {\rm H} $ & $2 \times 10^{-8} $\\

  ${\rm C}^+ + {\rm e} \longrightarrow {\rm C} +  h\nu $ & $4.4 \times 10^{-12} (300/T)^{0.61} $\\
  ${\rm m}^+ + {\rm e} \longrightarrow {\rm m} +  h\nu $ & $2.0 \times 10^{-7} (300/T)^{0.75} $\\
  ${\rm Mg}^+ + {\rm e} \longrightarrow {\rm Mg} +  h\nu $ & $2.8 \times 10^{-12} (300/T)^{0.86} $\\
     \hline
  ${\rm e} + G(0) \longrightarrow G(-) $&  $\pi a^2 \sqrt{\frac{8 k_B T}{\pi m_e }}(1)$\\
  ${\rm H^+} + G(0) \longrightarrow G(+) $&  $\pi a^2 \sqrt{\frac{8 k_B T}{\pi m_p }} ( 1)$\\
  ${\rm H_3^{+}} + G(0) \longrightarrow G(+) $&  $\pi a^2 \sqrt{\frac{8 k_B T}{3\pi m_p }} ( 1)$\\
  ${\rm He^{+}} + G(0) \longrightarrow G(+) $&  $\pi a^2 \sqrt{\frac{8 k_B T}{4\pi m_p }} ( 1)$\\
      \hline
${\rm e} + G(+) \longrightarrow G(0) $&  $\pi a^2 \sqrt{\frac{8 k_B T}{\pi m_e }}(1+\frac{\rm e^2}{a k_B T})$\\
  ${\rm H^{+}} + G(-) \longrightarrow G(0) + {\rm H} $&  $\pi a^2 \sqrt{\frac{8 k_B T}{\pi m_p }}(1+\frac{\rm e^2}{a k_B T})$\\

  ${\rm H_3^{+}} + G(-) \longrightarrow G(0) + {\rm H_2} + {\rm H} $&  $\pi a^2 \sqrt{\frac{8 k_B T}{3\pi m_p }}(1+\frac{\rm e^2}{a k_B T})$\\

  ${\rm He^{+}} + G(-) \longrightarrow G(0) + {\rm He}  $&  $\pi a^2 \sqrt{\frac{8 k_B T}{4\pi m_p }}(1+\frac{\rm e^2}{a k_B T})$\\
      \hline
$G(-) + G(+) \longrightarrow G(0) $&  $\pi (2a)^2 \sqrt{\frac{8 k_B T}{\pi \mu_g }}(1+\frac{\rm e^2}{2a k_B T})$\\
      
\end{tabular}
%\end{ruledtabular}
\end{table}



==> table_stick.tex <==
\begin{table}
\caption {Electron sticking coefficients $S(T, Z)$. 
Adapted from the Table 3 in \citep{grassi19}}
\label{ch_table_stick}
%\begin{ruledtabular}
\begin{tabular}{llllll}
  $Z$  & $c_{Z,1}$ &  $c_{Z,2}$ &  $c_{Z,3}$ \\
        \hline
  -1 & -0.39206456 & 0.26730250 & 0.16134104\\
   0 & -0.36848365 & 0.22498770 & 0.05100280\\
  +1 & -0.34350388 & 0.21428663 &-0.17200160\\
  +2 & -0.33385135 & 0.31951247 &-0.60550265
\end{tabular}
%\end{ruledtabular}
\end{table}
